Towards Open-Vocabulary Semantic Segmentation Without Semantic Labels

Large-scale vision-language models like CLIP have demonstrated impressive open-vocabulary capabilities for image-level tasks, excelling in recognizing what objects are present. However, they struggle with pixel-level recognition tasks like semantic segmentation, which additionally require understanding where the objects are located. In this work, we propose a novel method, PixelCLIP, to adapt the CLIP image encoder for pixel-level understanding by guiding the model on where, which is achieved using unlabeled images and masks generated from vision foundation models such as SAM and DINO. To address the challenges of leveraging masks without semantic labels, we devise an online clustering algorithm using learnable class names to acquire general semantic concepts. PixelCLIP shows significant performance improvements over CLIP and competitive results compared to caption-supervised methods in open-vocabulary semantic segmentation. Project page is available at https://cvlab-kaist.github.io/PixelCLIP

==> tex/figures/qual.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{tex/figures/ade.pdf}
  \caption{\textbf{Visualization on ADE-20K.}  We provide qualitative comparison on ADE-20K.}
  \label{fig:ade}
\end{figure}

==> tex/figures/qual_clusters.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{tex/figures/qual_clusters.pdf}
  \caption{\textbf{Visualization of inferencing with learned class prompts.}  We provide visualization of images inferenced with our learned class prompts for varying $k$. We observe that having larger $k$ values show more fine-grained, detailed recognition of the given images.}
  \label{fig:cluster_qual}
\vspace{-10pt}
\end{figure}

==> tex/figures/qualitative.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{tex/figures/fig1.pdf}
  \caption{\textbf{Illustration of different approaches.}  In contrast to existing methods utilizing image-text pairs as supervision, we utilize unlabeled masks as supervision for fine-tuning tuning the image encoder of CLIP. Moreover, through leveraging a shallow, light-weight mask decoder, we enforce the image encoder of CLIP to achieve dense vision-language alignment between image patches and text token.}
  \label{fig:illustration}
  \vspace{-10pt}
\end{figure}

==> tex/figures/teaser.tex <==
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{tex/figures/teaser.pdf}

\vspace{-10pt}
\caption{\textbf{ Overview of our method.} We propose PixelCLIP, a framework for fine-tuning the image encoder of CLIP~\cite{radford2021learning} with supervision from unlabeled masks \textit{without} reliance on any text data. Through leveraging high-quality unlabeled masks generated from segmentation foundation models~\cite{kirillov2023segment}, we learn dense representation that enables robust and precise vision-language alignment.
}
\label{fig:teaser}
\vspace{-25pt}
\end{figure}

==> tex/tables/ablation2.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablation studies}. We show results on open-vocabulary semantic segmentation for validating our design choices. We also report results from CLIP as baseline in the results.}
\label{tab:ablations}
%\vspace{-10pt}
\begin{subtable}{0.48\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
 %\multirow{2}{*}{A} &  \multirow{2}{*}{B} & \multicolumn{3}{c}{Evaluation Dataset}\\
 \multirow{2}{*}{$k$} & \multicolumn{5}{c}{Evaluation Dataset}\\
 &COCO & ADE-150 & Context59 & CityScapes & VOC\\
\midrule
Baseline~\cite{cherti2023reproducible} & 12.8 & 13.1 & 16.5 & 16.2 & 34.8\\ 
\midrule
32 & 19.8 & 19.4 & 33.0 & \underline{31.3} & 60.5 \\
\textbf{64} & \underline{21.1} & 20.2 & \textbf{34.2} & \textbf{33.2} & \textbf{66.0} \\
128 & 21.0 & \underline{20.3} & 33.5 & 30.1 & \underline{64.1} \\
256 & \textbf{21.3} & \textbf{20.4} & \underline{33.6} & 30.0 & \underline{64.1} \\

  \bottomrule
\end{tabular}
}
\caption{\textbf{Number of clusters.} For varying $k$, we find that scaling $k$ larger than 64 does not show much improvements, while $k=32$ also show competitive results.}
\label{tab:sub3}
\end{subtable}
%\hfill
\quad
% Subtable 1
\begin{subtable}{0.48\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
 %\multirow{2}{*}{A} &  \multirow{2}{*}{B} & \multicolumn{3}{c}{Evaluation Dataset}\\
 \multirow{2}{*}{$l$} & \multicolumn{5}{c}{Evaluation Dataset}\\
 &COCO & ADE-150 & Context59 & CityScapes & VOC\\
\midrule
Baseline~\cite{cherti2023reproducible} & 12.8 & 13.1 & 16.5 & 16.2 & 34.8\\ 
\midrule
1 & 20.2 & \underline{19.7} & 32.7 & 30.8 & \underline{64.5} \\
\textbf{4} & \underline{21.1} & \textbf{20.2} & \textbf{34.2} & \underline{33.2} & \textbf{66.0} \\
10 & \underline{20.4} & 19.6 & \underline{33.2} & 30.2 & 63.3 \\
20 & 19.9 & \underline{19.7} & 32.6 & \textbf{33.8} & 62.8 \\

  \bottomrule
\end{tabular}
}
\caption{\textbf{Length of learnable prompt token.} For varying $l$, we find that $l=4$ shows best overall performance.}
\label{tab:sub1}
\end{subtable}
%\quad % Adjust space between subtables here

\hfill

\begin{subtable}{0.48\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
 %\multirow{2}{*}{A} &  \multirow{2}{*}{B} & \multicolumn{3}{c}{Evaluation Dataset}\\
 \multirow{2}{*}{Moment.} & \multicolumn{5}{c}{Evaluation Dataset}\\
 &COCO & ADE-150 & Context59 & CityScapes & VOC\\
\midrule
Baseline~\cite{cherti2023reproducible} & 12.8 & 13.1 & 16.5 & 16.2 & 34.8\\ 
\midrule
\xmark & 17.8 & 17.0 & 25.6 & 23.3 & 51.6 \\
\checkmark & \textbf{21.1} & \textbf{20.2} & \textbf{34.2} & \textbf{33.2} & \textbf{66.0} \\
  \bottomrule
\end{tabular}
}

\caption{\textbf{Momentum Update.} Updating the mask encoder $E_M^V$ with momentum shows large gains as CLIP is initially not well-aligned to dense predictions. }
\label{tab:sub3}
\end{subtable}
%\hfill
\quad
% Subtable 1
\begin{subtable}{0.48\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
 \multirow{2}{*}{Text.} & \multicolumn{5}{c}{Evaluation Dataset}\\
 &COCO & ADE-150 & Context59 & CityScapes & VOC\\
\midrule
Baseline~\cite{cherti2023reproducible} & 12.8 & 13.1 & 16.5 & 16.2 & 34.8\\ 
\midrule
Fixed & 19.5 & 17.7 & 30.0 & 24.8 & 63.3 \\
$f_C$(Ours) & \textbf{21.1} & \textbf{20.2} & \textbf{34.2} & \textbf{33.2} & \textbf{66.0}\\

  \bottomrule
\end{tabular}
}
\caption{\textbf{Effects of utilizing learnable classes.} We compare our method of learnable class prompts to having pre-defined set of classes from COCO-Stuff~\cite{caesar2018coco}.}
\label{tab:sub1}
\end{subtable}

\end{table}


==> tex/tables/assoc.tex <==


\begin{table}[t]
\centering
\caption{\textbf{Results on Class Associativity.} We show results for predicting with learned class prompts, then mapping the results to classes in the dataset with the highest similarity to the prompt.}
\label{tab:assoc}
%\vspace{-10pt}
\begin{subtable}{0.48\textwidth}
\centering
\resizebox{\linewidth}{!}{
  \begin{tabular}{l|c|ccccc}
    \toprule
\multirow{2}{*}{$k$} &  \multicolumn{5}{c}{Evaluation Dataset}\\
 & Text&  COCO-St. & ADE-150 & Context & CityScapes & VOC\\
\midrule
 64& Learned & 3.2 & 3.4 & 12.3 & 14.3 & 20.1 \\
 64& Class & 21.1 & 20.2 & 33.3 & 30.1 & 64.6 \\
  \bottomrule
  \end{tabular}}
\caption{\textbf{$k=64$}}
\label{tab:sub3}
\end{subtable}
%\hfill
\quad
% Subtable 1
\begin{subtable}{0.48\textwidth}
\centering
\resizebox{\linewidth}{!}{
  \begin{tabular}{l|c|ccccc}
    \toprule
\multirow{2}{*}{$k$} &  \multicolumn{5}{c}{Evaluation Dataset}\\
 & Text&  COCO-St. & ADE-150 & Context & CityScapes & VOC\\
\midrule
128& Learned & 4.7 & 6.1 & 15.5 & 19.7 & 21.8 \\
128& Class & 21.1 & 20.2 & 32.8 & 30.1 & 64.9 \\

  \bottomrule
  \end{tabular}}
\caption{\textbf{$k=128$}.}
\label{tab:sub1}
\end{subtable}
%\quad % Adjust space between subtables here
\vspace{-20pt}
\end{table}


==> tex/tables/finetune.tex <==

\begin{table}[t]
  \caption{Quantitative comparison on open-vocabulary semantic segmentation. *Images were seen during training.
  }
  \vspace{-10pt}
  \label{tab:fine-tune}
  \centering
\resizebox{\linewidth}{!}{
  \begin{tabular}{l|c|c|cc|c|ccccc}
    \toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Training Dataset} & Total & \multicolumn{2}{c|}{Annotation} & Additional & \multicolumn{5}{c}{Evaluation Dataset}\\
 & &Images & Text & Mask & Parameters &  Stuff & ADE-150 & Context59 & CityScapes & VOC\\
\midrule
\midrule

\multicolumn{2}{l}{\textit{Without pre-trained VLMs}}\\
GroupViT~\cite{?}& CC12M, YFCC15M& 27M &\checkmark & \xmark & - & 24.3 & - & 22.4 & - & 52.3 \\
SegCLIP~\cite{?}& COCO, CC-12M& 12M & \checkmark & \xmark &\checkmark & 26.5 & - & 24.7 & - & 52.6 \\
\midrule
\multicolumn{2}{l}{\textit{With pre-trained VLMs}}\\
ReCo~\cite{?}& GCC12M& 12M & \checkmark & \xmark &\checkmark & 26.3 & - & 26.6 & 19.3 & - \\
TCL~\cite{?}& CC3M, CC12M& 15M&\checkmark & \xmark &\checkmark & 19.6 & 14.9 & 30.3 & 23.1 & 77.5 \\
SegCLIP~\cite{?}& COCO, CC-12M& 12M & \checkmark & \xmark &\checkmark & \phantom{0}\textcolor{gray}{26.5}* & - & 24.7 & - & 52.6 \\
PACL~\cite{?}& CC3M, CC12M, YFCC15M& 30M & \checkmark & \xmark &\checkmark & 38.8 & 31.4 & 50.1 & - & 72.3 \\

\midrule
 \hlrow(Ours)&  10\% SA-1B & 1.1M &\xmark & \checkmark & \xmark & 23.9 & 22.2 & 37.9 & 30.1 & 77.0 \\
  \bottomrule
  \end{tabular}}

\end{table}

==> tex/tables/main_table.tex <==

\begin{table}[t]
  \caption{Quantitative comparison on zero-shot semantic segmentation with vision-lanuage encoders only. }
  \vspace{-10pt}
  \label{tab:main_table}
  \centering
\resizebox{\linewidth}{!}{
  \begin{tabular}{l|c|c|ccccc}
    \toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Training Dataset} & \multicolumn{5}{c}{Evaluation Dataset}\\
 & & & 
COCO & ADE-150 & Context59 & CityScapes & VOC\\
\midrule
\midrule

CLIP~\cite{?}&   ViT-B/16 &WIT-400M~\cite{?} &  13.1 & 16.1 & 24.9 & 15.3 & 71.5 \\
SigLIP*~\cite{?}&   ViT-B/16 & WebLI~\cite{?} & 13.4 & 13.6 & 22.9 & 20.8 & 64.7 \\
SILC-C~\cite{?}&   ViT-B/16 & WebLI~\cite{?} & 20.8 & 19.3 & 31.6 & 26.9 & 77.5 \\
CLIP~\cite{?}&   ConvNeXt-B &LAION-2B~\cite{?} &  12.8 & 13.1 & 16.5 & 16.2 & 34.8 \\
\midrule
\hlrow \ours(Ours)&  ConvNeXt-B & 10\% SA-1B  & 21.1 (+0.0) & 20.2 (+0.0) & 33.3 (+0.0) & 30.1 (+0.0) & 64.5 (+0.0) \\
\midrule
CLIP~\cite{?}&   ViT-L/14 &WIT-400M~\cite{?} &  12.9 & 13.9 & 18.8 & 13.3 & 78.3 \\
CLIP~\cite{?}&   ConvNeXt-L &LAION-2B~\cite{?} &  16.9 & 15.2 & 22.9 & 17.1 & 57.2 \\
% SPARC~\cite{?}&   ViT-L & LAION-2B~\cite{?} & 16.5 & 22.2 & 21. & 30.1 & 77.0 \\
\midrule
 \hlrow \ours(Ours)&  ConvNeXt-L & 10\% SA-1B  & 24.5 (+8.0) & 22.5 (+0.0) & 38.2 (+0.0) & 30.5 (+0.0) & 77.7 (+0.0) \\
  \bottomrule
  \end{tabular}}

\end{table}
